Andromeda XXI -- a dwarf galaxy in a low density dark matter halo

Andromeda XXI (And XXI) has been proposed as a dwarf spheroidal galaxy with a central dark matter density that is lower than expected in the Standard $\Lambda$ Cold Dark Matter ($\Lambda$CDM) cosmology. In this work, we present dynamical observations for 77 member stars in this system, more than doubling previous studies to determine whether this galaxy is truly a low density outlier. We measure a systemic velocity of $v_r=-363.4\pm1.0\,{\rm kms}^{-1}$ and a velocity dispersion of $\sigma_v=6.1^{+1.0}_{-0.9}\,{\rm kms}^{-1}$, consistent with previous work and within $1\sigma$ of predictions made within the modified Newtonian dynamics framework. We also measure the metallicity of our member stars from their spectra, finding a mean value of ${\rm [Fe/H]}=-1.7\pm0.1$~dex. We model the dark matter density profile of And~XXI using an improved version of \GravSphere, finding a central density of $\rho_{\rm DM}({\rm 150 pc})=2.7_{-1.7}^{+2.7} \times 10^7 \,{\rm M_\odot\,kpc^{-3}}$ at 68\% confidence, and a density at two half light radii of $\rho_{\rm DM}({\rm 1.75 kpc})=0.9_{-0.2}^{+0.3} \times 10^5 \,{\rm M_\odot\,kpc^{-3}}$ at 68\% confidence. These are both a factor ${\sim}3-5$ lower than the densities expected from abundance matching in $\Lambda$CDM. We show that this cannot be explained by `dark matter heating' since And~XXI had too little star formation to significantly lower its inner dark matter density, while dark matter heating only acts on the profile inside the half light radius. However, And~XXI's low density can be accommodated within $\Lambda$CDM if it experienced extreme tidal stripping (losing $>95\%$ of its mass), or if it inhabits a low concentration halo on a plunging orbit that experienced repeated tidal shocks.

==> mnras/README <==
% readme.txt
%
% MNRAS journal LaTeX package
% v3.0 for LaTeX 2e
%
%
% This work may be distributed and/or modified under the
% conditions of the LaTeX Project Public License, either version 1.3
% of this license or (at your option) any later version.
% The latest version of this license is in
%   http://www.latex-project.org/lppl.txt
% and version 1.3 or later is part of all distributions of LaTeX
% version 2005/12/01 or later.
%
% This work has the LPPL maintenance status `author-maintained'.
% 
% The Current Maintainer of this work is: Royal Astronomical Society,
% MNRAS Editorial Office, who can be contacted on mn@ras.org.uk
%
% This work consists of all the files listed in readme.txt
%
%
% Last updated 22 May 2015
%
% Copyright (C) Royal Astronomical Society 2015, Blackwell Science 2001,
% Cambridge University Press 1994
%
% See each file for a detailed author list and change log.
%
% This package consists of the following files:

readme.txt          This file

mnras.cls           MNRAS LaTeX document class
mnras.bst           MNRAS BibTeX style

mnras_guide.tex     User guide, LaTeX format
mnras_guide.pdf     User guide, PDF format
mnras_template.tex  A simple template paper

example.eps         An example image used in the guide
example.png         An example image used in the guide
example.ps          An example image used in the guide

legacy\legacy.txt   Description of the legacy releases
legacy\mn2e.cls     v2.2 of mn2e.cls (deprecated)
legacy\mn2e.bst     v1.1b of mn2e.bst (deprecated)


% Disclaimer:
%
% This LaTeX package is provided free to the community in the hope that it
% assists them in preparing papers for the journal Monthly Notices of the
% Royal Astronomical Society.
% The files are provided 'as-is' with no guarantee of their suitability,
% freedom from errors or omissions, or compatibility with any software.
% The Royal Astronomical Society cannot provide user support for this package,
% LaTeX, or for any other software.
% Authors are free to use other styles or programmes if they wish.
% Please see the journal instructions to authors for guidance.
% This disclaimer is in addition to the No Warranty section of the licence,
% at the link given above.
